The devil is in the details: Enhancing Video Virtual Try-On via Keyframe-Driven Details Injection

Although diffusion transformer (DiT)-based video virtual try-on (VVT) has made significant progress in synthesizing realistic videos, existing methods still struggle to capture fine-grained garment dynamics and preserve background integrity across video frames. They also incur high computational costs due to additional interaction modules introduced into DiTs, while the limited scale and quality of existing public datasets also restrict model generalization and effective training. To address these challenges, we propose a novel framework, KeyTailor, along with a large-scale, high-definition dataset, ViT-HD. The core idea of KeyTailor is a keyframe-driven details injection strategy, motivated by the fact that keyframes inherently contain both foreground dynamics and background consistency. Specifically, KeyTailor adopts an instruction-guided keyframe sampling strategy to filter informative frames from the input video. Subsequently,two tailored keyframe-driven modules, the garment details enhancement module and the collaborative background optimization module, are employed to distill garment dynamics into garment-related latents and to optimize the integrity of background latents, both guided by keyframes.These enriched details are then injected into standard DiT blocks together with pose, mask, and noise latents, enabling efficient and realistic try-on video synthesis. This design ensures consistency without explicitly modifying the DiT architecture, while simultaneously avoiding additional complexity. In addition, our dataset ViT-HD comprises 15, 070 high-quality video samples at a resolution of 810*1080, covering diverse garments. Extensive experiments demonstrate that KeyTailor outperforms state-of-the-art baselines in terms of garment fidelity and background integrity across both dynamic and static scenarios.

==> secs/2_related_works.tex <==
\section{Related Work} 
\label{sec:related_work}
Video virtual try-on (VVT) aims to replace a person's clothing with a target garment while preserving the spatiotemporal consistency of the video, i.e., the generated results should ensure a consistent appearance of the target garment across frames, align seamlessly with the person’s pose and motion, and maintain the rest of the scene without distortion. 

%
Earlier works adopt GAN-based generators for VVT~\citep{dong2019fw,choi2021viton,zhong2021mv,jiang2022clothformer}. For instance, FW-GAN~\citep{dong2019fw}, as the first attempt, introduces an optical flow–guided warping GAN to deform the target garment and align it with the character’s body, thereby generating coherent video frames. 
MV-TON~\citep{zhong2021mv} leverages memory refinement to enhance details from previously generated frames. ClothFormer~\citep{jiang2022clothformer} employs a dual-stream transformer to address the temporal consistency of warped input sequences. 
%
Inspired by the advances of diffusion models in video generation~\citep{blattmann2023stable,wan2025wan,kong2024hunyuanvideo}, the latest studies~\citep{fang2024vivid,chong2025catv2ton,xu2024tunnel,zheng2024dynamic} have delved deeper into developing diffusion model–based frameworks for solving VVT tasks. 
%
For instance, ViVid~\citep{fang2024vivid} and Tunnel Try-on~\citep{xu2024tunnel} incorporate a clothing reference branch into the stable diffusion framework to inject appearance features of the target garment. They further introduce temporal modeling strategies to ensure temporal coherence across frames, achieving visually plausible and temporally consistent video generation. However, these pioneering methods treat spatial and temporal information separately and are limited to low-quality outputs due to the restricted expressive capacity of U-Net~\citep{unet} backbones.
%
To achieve superior realism and fine-grained detail preservation in virtual try-on applications, subsequent efforts~\citep{chong2025catv2ton,li2025magictryon,zuo2025dreamvvt} have explored diffusion transformer (DiT)–based diffusion models. These methods typically adopt a dual-branch architecture, where a dedicated clothing branch encodes appearance features, which are then combined with other input conditions and fed into DiT blocks for garment transfer. The DiT structure facilitates the joint modeling of spatial and temporal consistency. Furthermore, additional interaction modules are incorporated into the DiT blocks to better preserve garment details.

%
Despite the significant advancements of these DiT-based methods, they still suffer from limitations in fully capturing garment dynamics and background details. Furthermore, the introduction of additional components into DiT blocks often leads to increased complexity and computational overhead. Finally, the broader applicability of the DiT architecture remains constrained by the limited scale of publicly available datasets for virtual try-on tasks.
%
Our \M~offers a more lightweight solution that improves garment fidelity and background consistency by injecting keyframe-driven details without explicitly modifying the DiT architecture. In addition, we curate a large-scale, high-quality dataset \D, to address the issue of data scarcity.


% However, adapting such frameworks to DiT architectures presents new challenges. Compared to UNet-based backbones, DiTs involve significantly more parameters and computational cost~\citep{peebles2023scalable}. Moreover, integrating the clothing reference information at each frame exacerbates the burden in both memory and computation, making it difficult to scale such approaches to high-resolution video virtual try-on tasks.




% \textbf{Diffusion Model for Video Generation}
% With the continuous development of diffusion-based image synthesis techniques~\citep{rombach2022high,esser2024scaling,flux2024}, numerous frameworks have been proposed to extend diffusion models to the field of video generation~\citep{blattmann2023stable,wan2025wan,kong2024hunyuanvideo}. The architectures of diffusion-based generative methods can be broadly categorized into two types: UNet architecture and Transformer architecture. 
% Stable Video Diffusion~\citep{blattmann2023stable} extends Stable Diffusion~\citep{rombach2022high} by incorporating temporal modeling mechanisms such as temporal attention~\citep{wu2023tune} and 3D convolutions~\citep{tran2015learning}, thereby enhancing frame consistency and content coherence across video sequences. Wan employs a 3D causal variational autoencoder (VAE)~\citep{polyak2024movie,yang2024cogvideox} to capture complex temporal dynamics and extends the Diffusion Transformer (DiT) architecture from the image domain to the video domain, thereby achieving high-quality and temporally consistent video synthesis. 



==> secs/3_dataset_methodv2.tex <==
\section{\D~Dataset}
% To date, only two public virtual try-on datasets are available for video virtual tryon task: VVT~\citep{dong2019fw} and ViViD~\citep{fang2024vivid}. VVT dataset contains 791 videos and their corresponding garment images at a resolution of 256 $ \times $ 192. However, it includes only upper-body clothing, and the video content is highly repetitive, mostly limited to runway scenes. Due to its extremely low resolution, VVT lacks fine-grained texture and detail information of garments. As a result, evaluating methods on this dataset has become increasingly ineffective. With continuous improvements in model capabilities, performance metrics on VVT tend to saturate, making it difficult to distinguish genuine algorithmic improvements from fluctuations due to training stochasticity.

Currently, only two datasets--VVT~\citep{dong2019fw} and ViViD~\citep{fang2024vivid}--are available to support the VVTON task. Herein, VVT suffers from extremely low resolution, leading to the loss of fine-grained garment textures and details. Additionally, VVT is also restricted to simple, repetitive runway scenes. In contrast, ViViD provides higher resolution and greater scene diversity, yet its limited scale still falls short of the growing need for large, high-quality video–garment pairs driven by recent advances in DiT-based methods. Thus, in this work, we introduce a new dataset, named \D, which aims to significantly expand the currently available public datasets in both scale and quality. \NED{Table~\ref{tab:data_comp} provides a detailed comparison between our dataset and existing ones. Our proposed \D~contains 15,070 data samples, where each sample is at a resolution of $810 \times 1080$.}
\begin{table}[h]
\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{1}{c|}{\textbf{Datasets}} & \multicolumn{1}{c|}{\textbf{Resulotion}} & \multicolumn{1}{c|}{\textbf{Multi Class}} & \multicolumn{1}{c|}{\textbf{No Start Overexposure}}& \multicolumn{1}{c|}{\textbf{Subject Integrity}} & \multicolumn{1}{c}{\textbf{Pairs}}  \\ 
\midrule
VVT & $192\times256$ & \texttimes & \checkmark & \texttimes & 791\\
ViViD &  $632\times824$ & \checkmark & \texttimes & \texttimes & 9,700 \\
Ours & $810\times1080$ & \checkmark & \checkmark & \checkmark & 15,070 \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\caption{%
    \textbf{Datasets Comparison.} Compare the dataset with existing video virtual try-on datasets in terms of data modality, video content quality, resolution, and data scale.
}
\label{tab:data_comp}
\vspace{-10pt}
\end{table}

% This effort addresses the growing demand for larger-scale datasets driven by recent advances in model architectures.

\noindent \textbf{Data collection and processing}: Our raw data are downloaded from multiple e-commerce platforms. Each raw data sample consists of a high-resolution garment image together with a corresponding high-definition model showcase video, both cropped at a resolution of $1080 \times 810$. Then, for each raw data sample, we follow ViViD~\citep{fang2024vivid} to extract its pose video and masked video. Specifically, we employ OpenPose~\citep{cao2019openpose} to detect skeletal keypoints and generate pose sequences. To obtain masked videos, we adopt the same segmentation pipeline as OOTDiffusion~\citep{xu2025ootdiffusion}. For each frame, we utilize OpenPose~\citep{cao2019openpose} together with HumanParsing~\citep{li2020self} to infer body-part masks and create a garment-agnostic background image by inpainting the clothed regions. The resulting frames are then post-processed and stitched together to form the masked video. Furthermore, we categorize each data sample into one of three types--upper-body, lower-body, or full-body outfits--using BLIP-2~\citep{blip2}. During the data processing stage, we discard videos that contain a large number of frames with incomplete clothing occlusion to preserve subject integrity. In addition, we remove overexposed frames at the beginning of the original videos to maintain consistent color tones across all frames within each video. Finally, each input sample is composed of a reference garment image, the original showcase video, the pose video, and the masked video, along with its label. Fig.~\ref{fig:data} illustrates representative samples from each category of \D. 


% In response to this growing demand for high-quality and large-scale data, we introduce the XXX dataset, a new benchmark for virtual try-on. As shown in Table 1, the XXX dataset contains  video-clothing pairs at a resolution of $1080 \times 810$, making it the largest and highest-resolution virtual try-on dataset to date.


% Specifically, a motion video captures a person wearing the corresponding outfit performing comprehensive movements in an indoor environment, including turning, close-up views, walking, and other diverse actions. 



% Each raw data pair consists of a high-resolution front-view image of the garment with rich texture and detail, along with a motion video capturing a person wearing the corresponding outfit performing comprehensive movements in an indoor environment, including turning, close-up views, walking, and other diverse actions.



% Based on the raw data, we annotated the clothing categories into three types — upper-body, lower-body, and full-body outfits — following the format adopted by ViViD~\citep{fang2024vivid}. This annotation scheme facilitates easy adoption by the research community and ensures compatibility with existing virtual try-on frameworks.

% Among these, the pose video and masked video are essential for enabling the model to learn the visual relationship between human motion and clothing appearance, as well as to understand the interactions among the person, the clothing, and the background.

% \begin{figure}[ht]
% \centering
% \vspace{-8pt}
% \includegraphics[width=0.7\linewidth]{figs/data.pdf}
% \caption{\textbf{Data Illustration.} The dataset includes three categories of garments: upper-body, lower-body, and dresses. Each data sample consists of a garment reference image, the original video, an agnostic video, and a pose video.}
% \vspace{-10pt}
% \label{fig:data}
% \end{figure}

\begin{figure}[!ht]
\centering
\vspace{-8pt}
\subfigure[\textbf{Data Illustration.} The dataset includes three categories of garments: upper-body, lower-body, and dresses. Each data sample consists of a garment reference image, the original video, an agnostic video, and a pose video.]{
    \includegraphics[width=0.45\linewidth]{figs/data.pdf}
    \label{fig:data}
}
\hfill
\subfigure[\textbf{Distribution of Various Data Categories.}]{
    \includegraphics[width=0.45\linewidth]{figs/distribution1.pdf}
    \label{fig:distribution}
}
\vspace{-10pt}
\caption{Dataset overview. (a) Example data samples. (b) Distribution across garment categories.}
\label{fig:dataset_overview}
\end{figure}




% \begin{table*}[h]
% \vspace{-5pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \toprule
% \multicolumn{1}{c|}{\textbf{Datasets}} & \multicolumn{1}{c|}{\textbf{Resulotion}} & \multicolumn{1}{c|}{\textbf{Multi Class}} & \multicolumn{1}{c|}{\textbf{No Start Overexposure}}& \multicolumn{1}{c|}{\textbf{Subject Integrity}} & \multicolumn{1}{c|}{\textbf{Pairs}}& \multicolumn{1}{c|}{\textbf{Upper Body}}& \multicolumn{1}{c|}{\textbf{Lower Body}}& \multicolumn{1}{c}{\textbf{Dress}}  \\ 
% \midrule
% VVT & 192\times256 & \texttimes & \texttimes & \texttimes & 791 & 791 & - & -\\
% ViViD &  632\times824 & \checkmark & \texttimes & \texttimes & 9763 & 4824 & 2195 & 2744\\
% Ours & 810\times1080 & \checkmark & \checkmark & \checkmark & 15070 & 9629 & 3632 & 1809\\
% \bottomrule
% \end{tabular}
% }
% \vspace{-5pt}
% \caption{%
%     comparison
% }
% \label{tab:data_comp}
% \vspace{-10pt}
% \end{table*}



% In comparison, the ViViD dataset contains 9,700 video-clothing pairs with a resolution of 832 $ \times $ 624, covering three categories of clothing: upper-body, lower-body, and full-body outfits. It offers greater scene diversity and better supports a wide range of virtual try-on applications than VVT. However, as diffusion models based on the DiT architecture demonstrate increasing capabilities in video generation, the demands for both scale and quality of data in virtual try-on tasks have become more pronounced. Under these developments, ViViD is no longer sufficient to support the rapid progress of the field.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.95\linewidth]{figs/distribution.pdf}
% \caption{\textbf{Distribution of Various Data Categories.}}
% \label{fig:distribution}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \vspace{-8pt}
% \includegraphics[width=0.95\linewidth]{figs/data_comp.pdf}
% \caption{\textbf{Data.}}
% \vspace{-10pt}
% \label{fig:data_comp}
% \end{figure}




\section{Method}
Our method aims to lightweight existing dual-branch DiT-based \NED{VVTON} frameworks by adopting a single-branch design. The overall framework of our proposed \M~is illustrated in Fig.\ref{fig:pipeline}. \NED{Specifically, \M~first edits the initial frame of the source video using a pretrained image virtual try-on model, and then leverages the first-frame diffusion capability of a large-scale video DiT to generate the full video try-on.} This design reduces the heavy resource demands of video DiTs while preserving garment fidelity and multi-scale consistency. The details of \M~are elaborated in the remainder of this section.


% Our approach employs a single-branch framework, which only needs to inject garment appearance once into the latent input before diffusion-based generation. The overall framework of our proposed yyyyy is illustrated in Fig.\ref{fig:pipeline}. Speicifically, it first ... In the following sections, we will xxx

% Our method aims to edit the first frame using an image virtual try-on model, and then leverage the first-frame diffusion capability of a large-scale video DiT to achieve video virtual try-on. This approach addresses the high resource demands of video DiT when applied to the virtual try-on task. The overall framework of our proposed yyyyy is illustrated in Fig.\ref{fig:pipeline}.

\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\linewidth]{figs/pipeline.pdf}
\caption{\textbf{Overall framework of \M.} XXX leverages a pre-trained image virtual try-on model to inject garment appearance, and further adapts the input configuration on a LoRA-finetuned model to achieve a low-parameter, structure-preserving video virtual try-on strategy.}
\label{fig:pipeline}
\end{figure*}

\subsection{Instruction-guided Selection of Multi-view Keyframes}

% multi-anchor frames -> instruction-based

As we discussed in Sec.~\ref{sec:intro}, existing DiT-based frameworks adopt a dual-branch paradigm that repeatedly injects garment appearance features from the reference branch into the DiT backbone, resulting in substantial computational overhead. In addition, these methods require architectural adaptations of the backbone network to achieve better feature alignment, which further increase resource demands and model complexity. Consequently, reducing appearance feature injection frequency and minimizing structural modifications have become increasingly urgent to balance model efficiency and generation performance. \NED{To fulfill this goal, inspired by Wan’s~\citep{wan2025wan} highly harmonious performance in video content synthesis and considering that the noise input already encodes video structural information, we propose a novel garment appearance injection strategy based on first-frame editing, as illustrated in Fig.~\ref{fig:pipeline}.}




 % Existing approaches, largely inherited from image virtual try-on frameworks, adopt a dual-branch architecture. However, such designs introduce a unique challenge when applied to DiT: the repeated injection of garment appearance features from the reference branch into the backbone network, together with architectural adaptations, results in substantial computational overhead. This creates a critical trade-off between model efficiency and generation performance. Therefore, reducing the frequency of appearance feature injections and minimizing structural modifications are key to achieving efficient and effective video virtual try-on. Noticing Wan's highly harmonious performance in video content synthesis and the fact that the noise input contains video structure information, we propose a novel garment appearance injection strategy for the first frame, as illustrated in Fig.\ref{fig:pipeline}.



Specifically, given a reference garment image $r_{\text{gar}}$ and the garment-agnostic video $x_{\text{agn}}$ from the source video, we first extract the initial frame $i_{\text{agn}}^0$ from $x_{\text{agn}}$. We then employ a pre-trained image virtual try-on model $M_{\text{img}}$ to inject the garment appearance. Since

\begin{equation}
    i_{\text{inj}}^0 = M_{\text{img}}(i_0, c_i, r_{\text{gar}})
\end{equation}

% For $ i_0 $, which is an image virtual try-on task, existing image virtual try-on models have the capability to capture fine-grained garment texture details and handle person-clothing interactions effectively. Therefore, we employ a pretrained image virtual try-on model FiTDiT $ M_{\text{FiT}} $~\cite{jiang2024fitdit} to perform appearance injection on $ i_0 $, obtaining a high-quality image try-on result $ i_r $. The formal process is formulated as:
% \begin{equation}
    % i_r = M_{\text{FiT}}(i_0, c_i, r_{clo})
% \end{equation}
where $ c_i $ refers to the given textual instruction that uniformly describes the clothing change process, and $ r_{\text{clo}} $ denotes the front-view high-resolution image of the garment, serving as the source of detailed texture information for the clothing.

In order to minimize disruption to Wan's temporal priors in video synthesis and reduce information perturbation, we adopt Wan's image encoder $ E_{\text{img}} $ to obtain the latent space feature $ L_g $ of $ i_r $. 
Due to the edited first frame contains complete human skeletal structure, and accurate pose control is crucial for ensuring motion consistency in video virtual try-on tasks, we further employ Wan's VAE $ E_{vae} $ to obtain the latent representation $ L_p $ of the pose video $ v_p $. 
Subsequently, $ L_g $ is embedded as the first token into $ L_v $, resulting in a unified latent sequence $ L $ that incorporates both temporal dynamics and garment appearance information. The mathematical formulation is as follows:
\begin{equation}
L = R\left(\text{E}_{vae}(v_p),\ E_{\text{img}}(i_r)\right)
\end{equation}
where $ R $ denotes the embedding operation, and $ L \in \mathbb{R}^{N \times d} $.

% Similarly, for $ x'_{\text{agn}} $, we also reuse Wan's VAE to extract its latent representation $ L_v $. Subsequently, $ L_g $ is embedded as the first-frame token at the beginning of $ L_v $, resulting in a combined latent representation $ L $ that incorporates both temporal and garment appearance information. The mathematical formulation is as follows:
% \begin{equation}
%     L = R\left(\text{VAE}(x'_{\text{agn}}), E_{\text{img}}(i_r)\right)
% \end{equation}
% where $ R $ denotes the embedding operation, and $ L \in \mathbb{R}^{N \times d} $.

\begin{table}[h]
\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\multicolumn{1}{c|}{\textbf{Method}} &\multicolumn{1}{c|}{\textbf{Framework}} & \multicolumn{1}{c|}{\textbf{Reference Injection}} & \multicolumn{1}{c}{\textbf{No Structural Modifications}}  \\ 
\midrule
OOTDiffusion & dual branch & N & \texttimes \\
ViViD & dual branch &  N & \texttimes \\
CatV$^2$TON & dual branch & N & \texttimes \\
MagicTryOn & dual branch & N & \texttimes \\
Ours & single branch & 1 & \checkmark \\
\bottomrule
\end{tabular}}
\vspace{-5pt}
\caption{%
    \textbf{Method Complexity Analysis.} Analyze the complexity of method from two key perspectives: the number of garment appearance injection steps and whether the backbone network is modified during implementation.
}
\label{tab:condition_types}
\vspace{-10pt}
\end{table}
As shown in Table 2, the proposed architecture offers the following advantages: a): Previous dual-branch approaches require injecting garment appearance information at every time step, whereas the proposed single-branch architecture only needs a single injection at the input stage. b): The dual-branch architecture often requires modifications to the backbone network due to the need for aligning garment features with the latent feature space. In contrast, the proposed single-branch architecture effectively avoids such architectural changes.

Specifically, the garment appearance injection strategy in dual-branch architectures urgently requires an adaptation module to align the garment features with the latent features of the diffusion model. Moreover, to achieve more harmonious synthesis results and ensure cross-frame consistency of the garment features in the video, such methods often need to further modify the backbone architecture in order to project the garment features into the latent feature space of the backbone. We observe that the significant performance improvement of DiT over the UNet architecture allows DiT to leverage its powerful temporal priors to maintain both consistency and quality in video synthesis. Therefore, our strategy of injecting garment information only at the first frame avoids any modification to the backbone network architecture, while achieving a balanced trade-off between efficiency and temporal consistency.

\subsection{Preserving Background Integrity}
Since the pose video focuses on human motion estimation and eliminates scene information from clothing-agnostic regions, it inevitably loses the layout information of the background, which is a critical component for synthesizing realistic scenes in high-quality videos. In addition, maintaining low backbone perturbation while aligning with the garment appearance injection strategy is essential for improving model efficiency. To this end, we propose a lightweight background encoder to enhance the background information from the agnostic video, while avoiding any adaptation or modification to the backbone network.

The encoder $ E_m $ consists of four 3D convolutional layers, with channel dimensions of 32, 96, 192, and 256, respectively.  
To facilitate smoother guidance of the mask latent during training for video synthesis, we zero-initialize a linear layer within the mask guider. Specifically, as illustrated in Figure~4, the clothing-agnostic video $ x_{\text{agn}} $ is fed into the mask guider, and its output $ L_m $ is subsequently added to the input features concatenated at the second stage of the backbone network. The corresponding mathematical formulation is given as:
\begin{equation}
L = L + E_m(x_{\text{agn}}).
\end{equation}

To further reduce the number of trainable parameters when fine-tuning the diffusion model based on the DiT architecture, we apply LoRA to the backbone attention modules in Wan, including both the self-attention and cross-attention modules. The formulation is as follows:
\begin{equation}
\begin{aligned}
Q &= W_{Q} + A_Q B_Q^\top, \\
K &= W_{K} + A_K B_K^\top, \\
V &= W_{V} + A_V B_V^\top,
\end{aligned}
\end{equation}
where $ W_{Q}, W_{K}, W_{V} $ denote the pre-trained weight matrices of the original projection layers, and $ A_Q, B_Q, A_K, B_K, A_V, B_V $ are low-rank trainable matrices with rank $ r \ll \min(d, k) $. This parameter-efficient adaptation enables dynamic modulation of attention mechanisms while preserving the original model capacity. We further apply LoRA to the linear transformations in the feed-forward network (FFN), where each weight matrix $ W_{F0} $ is similarly parameterized as $ W_F = W_{F} + A_F B_F^\top $. This extension allows for lightweight fine-tuning across both attention and MLP components of the diffusion Transformer.

\begin{algorithm}[H]
    \caption{Instruction-Guided Multi-View Keyframe Sampling for Video Try-On}
    \KwIn{
        $V_{\text{in}}$: Input video (T frames, indices $0\sim T\!-\!1$ with timestamps $t_0\sim t_{T-1}$)\\
        $\text{Ins}$: User instruction (e.g., "Show front/back of clothes, raise hand to display sleeves")\\
        $\text{Params}$: 
        $K_{\text{max}}$ (max keyframes: 3 for short video, 6 for long video),\\
        $w_1\!=\!0.3, w_2\!=\!0.2, w_3\!=\!0.3, w_4\!=\!0.2$ (weight coefficients),\\
        $T_{\text{thres}}$ (temporal interval threshold: video duration/5),\\
        $\text{Occlu}_{\text{thres}}\!=\!0.2$ (garment occlusion threshold),\\
        $\lambda\!=\!0.5$ (skeleton difference weight)
    }
    \KwOut{$F_{\text{key}}$: Selected keyframe list (length $\leq K_{\text{max}}$)}

    % Step 1: Parse instruction
    $\text{View}_{\text{targets}}, \text{Action}_{\text{targets}} = \text{parse\_instruction}(\text{Ins})$ \;
    %\Comment{Extract target views (e.g., "front", "back") and actions (e.g., "raise\_hand") via VLM}

    % Step 2: Generate multi-anchor frames
    $F_{\text{anchor}} = []$ \;
    \For{each $\text{view} \in \text{View}_{\text{targets}}$}{
        $F_{\text{anchor}}.append(\text{generate\_standard\_pose}(\text{view}))$ \;
    }
    \For{each $\text{action} \in \text{Action}_{\text{targets}}$}{
        $F_{\text{anchor}}.append(\text{generate\_standard\_pose}(\text{action}))$ \;
    }
    $D_{\text{anchor}} = [\text{compute\_joint\_direction}(f) \mid f \in F_{\text{anchor}}]$ \;
    %\Comment{Multi-anchor frames instead of fixed single anchor (adapts to instruction)}

    % Step 3: Compute frame scores
    $S = []$ \;  % List of (frame_idx, timestamp, total_score)
    \For{$i = 0$ to $T\!-\!1$}{
        $f = V_{\text{in}}[i]$, $t = \text{timestamp of } f$ \;
        
        % Instruction matching score
        $S_{\text{ins}} = \text{vlm\_score}(f, \text{Ins})$ \;  % 0~1, higher = better match
        
        % Skeleton difference (distance to nearest anchor)
        $D_f = \text{compute\_joint\_direction}(f)$ \;
        $S_m = \min(\{\text{cosine\_distance}(D_f, d) \mid d \in D_{\text{anchor}}\})$ \;
        
        % Garment visibility score
        $\text{cloth\_mask} = \text{segment\_garment}(f)$ \;  % Garment region segmentation
        $S_{\text{cloth}} = \text{area}(\text{cloth\_mask}) / \text{area}(f)$ \;  % 0~1
        
        % Occlusion check (filter severely occluded frames)
        $\text{occlusion\_ratio} = \text{area}(\text{occluded\_region}(\text{cloth\_mask})) / \text{area}(\text{cloth\_mask})$ \;
        \If{$\text{occlusion\_ratio} > \text{Occlu}_{\text{thres}}$}{
            \Continue \;  % Skip frames with >20% garment occlusion
        }
        
        % Initial total score
        $\text{initial\_score} = w_1\!*\!S_{\text{ins}} + w_2\!*(1\!-\!S_m) + w_3\!*\!S_{\text{cloth}} + w_4\!*\!1.0$ \;
        $S.append((i, t, \text{initial\_score}))$ \;
    }
    %\Comment{Multi-dimensional scoring: instruction alignment + motion difference + visibility}

    % Step 4: Global selection with temporal uniformity
    $S_{\text{sorted}} = \text{sort}(S, \text{key}=\lambda x: x[2], \text{reverse=True})$ \;  % Sort by initial score
    $\text{Idx}_{\text{key}} = []$, $T_{\text{selected}} = []$ \;
    
    \For{each $(\text{idx}, t, \text{score}) \in S_{\text{sorted}}$}{
        \If{$|\text{Idx}_{\text{key}}| \geq K_{\text{max}}$}{
            \Break \;
        }
        
        % Temporal interval score (encourage uniform distribution)
        \If{$T_{\text{selected}}$ is empty}{
            $S_t = 1.0$ \;
        }
        \Else{
            $\text{min\_t\_dist} = \min(\{|\!t - t_s| \mid t_s \in T_{\text{selected}}\})$ \;
            $S_t = \text{min\_t\_dist} / T_{\text{thres}}$ \;  % Higher for larger intervals
        }
        
        % Final score with temporal adjustment
        $\text{final\_score} = \text{score} * S_t$ \;
        
        % Filter redundant frames
        \If{$\text{Idx}_{\text{key}}$ is empty}{
            $\text{Idx}_{\text{key}}.append(\text{idx})$ \;
            $T_{\text{selected}}.append(t)$ \;
        }
        \Else{
            $\text{min\_score\_diff} = \min(\{|\!\text{final\_score} - S[ik][2]| \mid ik \in \text{Idx}_{\text{key}}\})$ \;
            \If{$\text{min\_score\_diff} \geq 0.1$ and $\text{min\_t\_dist} \geq T_{\text{thres}}$}{
                $\text{Idx}_{\text{key}}.append(\text{idx})$ \;
                $T_{\text{selected}}.append(t)$ \;
            }
        }
    }
    %\Comment{Balance score and temporal uniformity (avoids redundancy in long videos)}

    % Output
    $F_{\text{key}} = [V_{\text{in}}[\text{idx}] \mid \text{idx} \in \text{Idx}_{\text{key}}]$ \;
    \Return $F_{\text{key}}$ \;
\end{algorithm}

% Algorithm 2: Instruction-Guided Multi-View Keyframe Sampling
% Input:
%   Vin: 输入视频（含T帧，帧索引0~T-1，时间戳t0~tT-1）
%   Ins: 用户指令（如“展示服装正面、背面，抬手显袖子弹性”）
%   Params:
%     K_max: 最大关键帧数（短视频K_max=3，长视频K_max=6）
%     w1~w4: 权重（w1=0.3, w2=0.2, w3=0.3, w4=0.2，可微调）
%     T_thres: 时间间隔阈值（如视频时长/5，确保关键帧均匀）
%     Occlu_thres: 服装遮挡率阈值（如20%，超过则排除）
%     λ: 骨骼差异权重（0.5）
% Output:
%   F_key: 最终关键帧列表（数量≤K_max）

% # 步骤1：指令解析（提取关键动作与目标视角）
% 1: 利用VLM（如Qwen2.5VL）解析Ins，输出：
%    - View_targets: 目标视角列表（如["front", "back", "side"]）
%    - Action_targets: 关键动作列表（如["raise_hand", "turn_around"]）

% # 步骤2：动态生成多锚帧（对应目标视角与动作）
% 2: 生成锚帧列表F_anchor：
%    For each view in View_targets:
%      生成该视角的标准姿势帧（如front→正面A姿，back→背面A姿）
%    For each action in Action_targets:
%      生成该动作的标准帧（如raise_hand→抬手姿势帧）
% 3: 计算所有锚帧的骨骼关节方向向量D_anchor = [compute_joint_dir(f) for f in F_anchor]

% # 步骤3：逐帧计算多维度分数
% 4: 初始化帧分数列表S = []
% 5: For each frame_idx in 0~T-1:
%    a. 提取当前帧f = Vin[frame_idx]，其时间戳t = t_frame_idx
%    b. 计算指令匹配度S_ins：
%       S_ins = VLM_score(f, Ins)  # 0~1，分数越高越匹配指令
%    c. 计算骨骼差异Sm：
%       D_f = compute_joint_dir(f)
%       Sm = min( [cosine_dist(D_f, d) for d in D_anchor] )  # 取与最近锚帧的差异（越小差异越大）
%    d. 计算服装区域占比S_cloth：
%       cloth_mask = saliency_segment(f, "garment")  # 服装分割（参考DreamVVT的3.2.1）
%       S_cloth = area(cloth_mask) / area(f)  # 服装面积/帧面积（0~1）
%    e. 计算服装遮挡率Occlu：
%       Occlu = area(occlusion_mask(cloth_mask)) / area(cloth_mask)  # 遮挡区域/服装面积
%    f. 若Occlu > Occlu_thres：跳过该帧（服装遮挡严重）
%    g. 计算综合分数S_total：
%       S_total = w1*S_ins + w2*(1-Sm) + w3*S_cloth + w4*initial_S_t  # (1-Sm)使差异大则分数高；initial_S_t初始为1
%    h. 将(frame_idx, t, S_total)加入S

% # 步骤4：全局筛选（按分数+时间均匀性）
% 6: 按S_total降序排序S → S_sorted
% 7: 初始化关键帧索引列表Idx_key = []，已选时间戳列表T_selected = []
% 8: For each (idx, t, score) in S_sorted:
%    a. 若len(Idx_key) ≥ K_max：break
%    b. 计算时间间隔得分S_t：
%       if T_selected is empty:
%           S_t = 1  # 第一帧无时间约束
%       else:
%           min_t_dist = min( [abs(t - ts) for ts in T_selected] )
%           S_t = min_t_dist / T_thres  # 时间差越大，S_t越高（0~1）
%    c. 更新当前帧最终分数：final_score = score * S_t
%    d. 若Idx_key为空：
%           Idx_key.append(idx)
%           T_selected.append(t)
%    e. Else：
%           # 确保分数差≥阈值（避免冗余）且时间间隔≥T_thres
%           min_score_diff = min( [abs(final_score - S[ik][2]) for ik in Idx_key] )
%           if min_score_diff ≥ 0.1 and min_t_dist ≥ T_thres:
%               Idx_key.append(idx)
%               T_selected.append(t)

% # 步骤5：输出关键帧
% 9: F_key = [Vin[idx] for idx in Idx_key]
% 10: return F_key

\subsection{Training Objective}
As shown in Figure 2, fine-tuning is conducted on both the LoRA parameters added to the DiT blocks and the parameters of the mask guider module, starting from pre-trained weights, with all other modules kept frozen. During fine-tuning, to optimize the learning of pose control, the input first frame is set to be the original first frame of the video, in order to eliminate any bias or misalignment between the output of the image virtual try-on model and the pose map produced by the pose estimator.

By leveraging flow matching to maintain equivalence with the maximum likelihood objective, the model is trained to learn the true velocity. The overall training objective $ \mathcal{L} $ is formulated as follows:
\begin{equation}
\mathcal{L} = \mathbb{E}_{c_{\text{txt}}, t, x_1, x_0} \left[ \| u(x_t, L, c_{\text{txt}}, t; \theta) - v_t \|_2^2 \right]
\end{equation}
where $ u(x_t, L, c_{\text{txt}}, t; \theta) $ denotes the output velocity predicted by the model.


